Ares: A System-Oriented Wargame Framework for Adversarial ML

Since the discovery of adversarial attacks against machine learning models nearly a decade ago, research on adversarial machine learning has rapidly evolved into an eternal war between defenders, who seek to increase the robustness of ML models against adversarial attacks, and adversaries, who seek to develop better attacks capable of weakening or defeating these defenses. This domain, however, has found little buy-in from ML practitioners, who are neither overtly concerned about these attacks affecting their systems in the real world nor are willing to trade off the accuracy of their models in pursuit of robustness against these attacks. In this paper, we motivate the design and implementation of Ares, an evaluation framework for adversarial ML that allows researchers to explore attacks and defenses in a realistic wargame-like environment. Ares frames the conflict between the attacker and defender as two agents in a reinforcement learning environment with opposing objectives. This allows the introduction of system-level evaluation metrics such as time to failure and evaluation of complex strategies such as moving target defenses. We provide the results of our initial exploration involving a white-box attacker against an adversarially trained defender.

==> outline.tex <==
\section{Outline}
\begin{itemize}
    \item Adv attacks exists. Many defenses have been proposed, but tend to break when adaptive white-box attacks are used
    \item However, white-box isn't a very great way to evaluate the attacks with respect to real attackers. While it would be great to have a defense that resists white-box, we might be throwing away defenses that could be useful in a more realistic scenario
    \item We are developing an evaluation framework to measure the time is takes for a PGD attacker to succeed in multiple different defender scenarios. We base our evaluation framework on the MTD structure. 
    \item  First, we re-examine effectiveness of such a framework on white-box attacks using different combinations non-AT and AT models to study the issue with such a defense structure. We find that, in general, the attacker always wins, but takes longer with AT models. Also, combining models of the same type does not drastically reduce the time for a successful attack.
    \item Based on prior work, we assume that the lack of effectiveness of the MTD (and by extension ensemble defense) is due to a shared attack gradient. We find that this is the case when we study the cosine sim for samples that multiple models fail or only a single model fails on.
    \item Future work: If we use training method that encourages diverse gradients, does it increase the time it takes for an attacker to succeed?
    \item Future work: When we switch to a blackbox threat model, how does this affect the time it takes for an attacker to succeed?
    \item Future work: When we use a blackbox threat model along with prior "broken" defenses, how does this affect the time it takes for an attacker to succeed?
    \item Future Work: Why does the defender need to stay silent? When we enable a detection defense for the attack (such as the PR in ART), how does this affect the attack success rate and the attacker's behavior?
    
    
\end{itemize}

\paratitle{Amir scratch board}
Unlike traditional evaluations, which typically focuses on measures of robustness, \sys allows researchers to take a system-oriented view at adversarial ML and examine 
